Jet energy measurement with the ATLAS detector in proton-proton collisions at sqrt(s) = 7 TeV

The jet energy scale (JES) and its systematic uncertainty are determined for jets measured with the ATLAS detector at the LHC in proton-proton collision data at a centre-of-mass energy of sqrt(s) = 7 TeV corresponding to an integrated luminosity of 38 inverse pb. Jets are reconstructed with the anti-kt algorithm with distance parameters R=0.4 or R=0.6. Jet energy and angle corrections are determined from Monte Carlo simulations to calibrate jets with transverse momenta pt > 20 GeV and pseudorapidities eta<4.5. The JES systematic uncertainty is estimated using the single isolated hadron response measured in situ and in test-beams. The JES uncertainty is less than 2.5% in the central calorimeter region (eta<0.8) for jets with 60 < pt < 800 GeV, and is maximally 14% for pt < 30 GeV in the most forward region 3.2<eta<4.5. The uncertainty for additional energy from multiple proton-proton collisions in the same bunch crossing is less than 1.5% per additional collision for jets with pt > 50 GeV after a dedicated correction for this effect. The JES is validated for jet transverse momenta up to 1 TeV to the level of a few percent using several in situ techniques by comparing a well-known reference such as the recoiling photon pt, the sum of the transverse momenta of tracks associated to the jet, or a system of low-pt jets recoiling against a high-pt jet. More sophisticated jet calibration schemes are presented based on calorimeter cell energy density weighting or hadronic properties of jets, providing an improved jet energy resolution and a reduced flavour dependence of the jet response. The JES systematic uncertainty determined from a combination of in situ techniques are consistent with the one derived from single hadron response measurements over a wide kinematic range. The nominal corrections and uncertainties are derived for isolated jets in an inclusive sample of high-pt jets.

==> atlasdetectorpicture.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htp!]
\begin{center}
\includegraphics[width=0.9\textwidth]{Atlasfigures/atlasdetector.eps} 
\vspace {-1.5cm}
\caption{
Sketch of the inner part of a quarter of the \ATLAS{} detector showing
the inner detector and the electromagnetic calorimeter.
The protons collide in the middle of the detector displayed as the left lower point.
From inner to outer are shown: the inner detector with the \Pixel, \SCT{} and the
\TRT{} tracking devices, the warm cryostat wall, 
the superconducting solenoid coil, 
the cold cryostat wall, the presampler and the liquid argon calorimeter.
Shown is the barrel and the endcap part of the detector.
The endcap part is split in an inner and an outer wheel.
Also displayed are the pseudorapidity ($\eta$) values measured for particles produced
at the nominal interaction point (dashed lines). The solid line
at the bottom indicates the spatial dimensions of the detector.
}
\label{fig:ATLASdetector}
\end{center}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> gsc-tracking-gammajet-figures.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht!]
\centering
\subfloat[\fpres]{\includegraphics[width=0.49\textwidth]{GSCfigures/GammaJet/GSsyst_gammaJets.eps}}
\caption{Ratio of the detector response in data and the \pythia{} MC10 sample using direct \pt{} balance 
in $\gamma$-jets events after \GS{} relative to \EMJES. The jets used have $|\etajet| < 1.2$.} 
\label{fig:GammaJet}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> jetenergyaftercalibration.tex <==
A basic jet-level validation of the more complex jet calibration schemes can be performed by looking 
at the differences in the energy of jets before and after the weighting is performed in both Monte Carlo simulation 
and data. As in the previous section, this provides a good measure of how the differences between data
and Monte Carlo simulation observed in other sections impact the size of the corrections applied to arrive
to the calibrated jet energy scale.

Figure~\ref{fig:EcalEemPt} shows the mean of the ratio of calibrated over uncalibrated jet energies as a 
function of calibrated jet $\pt$ for the \GS, \GCW{} and \LCW{} calibration schemes for jets with $|\rapjet|<0.3$.  
%-----------------------------------
% Ecal/Eem vs pT, eta
%-----------------------------------
\begin{figure}[!ht]
\begin{center}
\subfloat[Global sequential calibration]{
  \label{fig:EcalEemPt:1}
  \includegraphics[width=0.45\textwidth]{JetInputsfigures/fracEcalEem_vs_pt_comparisonDataMC_y_0_3_after3corr.eps}
}
\subfloat[Global cell-weighting calibration]{
  \label{fig:EcalEemPt:2}
 \includegraphics[width=0.45\textwidth]{JetInputsfigures/jetCalRatio_pt0_AntiKt6H1Topo.eps}% 
  }
\subfloat[Local cluster calibration]{
  \label{fig:EcalEemPt:3}
    \includegraphics[width=0.45\textwidth]{JetInputsfigures/jetCalRatio_pt0_AntiKt6LCTopoJES.eps}
}
\caption{Mean calibrated jet energy over uncalibrated jet energy as a function of calibrated jet $\pt$ for 
jets constructed of topological clusters calibrated with \subref{fig:EcalEemPt:1} 
the global sequential, \subref{fig:EcalEemPt:2} the global cell energy density weighting,
 and \subref{fig:EcalEemPt:3} local cluster weighting calibration schemes. The mean value is shown as obtained in data 
        (black points) and in Monte Carlo simulation (red open squares). 
}
\label{fig:EcalEemPt}
\end{center}
\end{figure}
%-----------------------------------
For the GS correction the width correction is not applied for the reasons stated in 
Section~\ref{sec:GSinputs}. In the Monte Carlo, all calibrations apply the same correction
factors on average, indicating that they all calibrate jets correctly.
The agreement between the factors applied in the data and the Monte Carlo simulation is better than 1\% for the GS calibration and better than 2\% for the others. The agreement becomes slightly worse for the GS calibration if the width correction is applied. 
This points to a reason why the other calibration schemes show 2\% level disagreements:
they may be implicitly considering variables that are correlated to the width distribution,
and are, thus, different in the data and the Monte Carlo simulation.
Figure~\ref{fig:EcalEemEta} shows the mean of the ratio of calibrated over uncalibrated jet energies as a function of rapidity for the GS, GCW and LCW calibration schemes for jets with calibrated jet $\pt$ above $20\GeV$.  
%-----------------------------------
\begin{figure}[!ht]
\begin{center}
\subfloat[Global sequential calibration]{
  \label{fig:EcalEemEta:1}
  \includegraphics[width=0.45\textwidth]{JetInputsfigures/AntiKt6Topo_r1206_ptcut20GeV/fracEcalEem_vs_eta_comparisonDataMC_after3corr.eps}}
\subfloat[Global cell-weighting calibration]{
  \label{fig:EcalEemEta:2}
  \includegraphics[width=0.45\textwidth]{JetInputsfigures/jetCalRatio_eta0_AntiKt6H1Topo.eps}
        }
\subfloat[Local cluster calibration]{
  \label{fig:EcalEemEta:3}
   \includegraphics[width=0.45\textwidth]{JetInputsfigures/jetCalRatio_eta0_AntiKt6LCTopoJES.eps}
}
\caption{ Mean calibrated jet energy over uncalibrated jet energy as a function of the rapidity for jets
         constructed of topological clusters calibrated with \subref{fig:EcalEemEta:1} the global sequential, 
\subref{fig:EcalEemEta:2} the global cell energy density weighting, and \subref{fig:EcalEemEta:3}
 local cluster weighting calibration schemes. 
The mean value is shown as obtained in data (black points) and in Monte Carlo simulation (red open squares).}
\label{fig:EcalEemEta}
\end{center}
\end{figure}
As in the previous figure, all calibrations apply the same correction
factors on average, in the Monte Carlo indicating that they all calibrate jets correctly. 
The agreement between the factors applied in the data and the Monte Carlo simulation is also better
 than 1\% for the GS calibration and better than 2\% for the other calibration schemes in the whole rapidity range. 


==> jetuncertaintycomparisonfiguresr4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htp]
\begin{center}
\subfloat[\etaRange{0}  {0.3}]{\includegraphics[width=0.4\textwidth]{InSituCombination/overlaidUncertainty_AKT4_0_0.3.eps}}
\subfloat[\etaRange{0.3}{0.8}]{\includegraphics[width=0.4\textwidth]{InSituCombination/overlaidUncertainty_AKT4_0.3_0.8.eps}}\\
\subfloat[\etaRange{0.8}{1.2}]{\includegraphics[width=0.4\textwidth]{InSituCombination/overlaidUncertainty_AKT4_0.8_1.2.eps}}
\subfloat[\etaRange{1.2}{2.1}]{\includegraphics[width=0.4\textwidth]{InSituCombination/overlaidUncertainty_AKT4_1.2_2.1.eps}}\\
\subfloat[\etaRange{2.1}{2.8}]{\includegraphics[width=0.4\textwidth]{InSituCombination/overlaidUncertainty_AKT4_2.1_2.8.eps}}
\subfloat[\etaRange{2.8}{3.2}]{\includegraphics[width=0.4\textwidth]{InSituCombination/overlaidUncertainty_AKT4_2.8_3.2.eps}}\\
\subfloat[\etaRange{3.2}{3.6}]{\includegraphics[width=0.4\textwidth]{InSituCombination/overlaidUncertainty_AKT4_3.2_3.6.eps}}
\subfloat[\etaRange{3.6}{4.5}]{\includegraphics[width=0.4\textwidth]{InSituCombination/overlaidUncertainty_AKT4_3.6_4.5.eps}}
%
\caption{%a) 
Fractional \JES{} uncertainties for \antikt{} jets with $R = 0.4$ for the various $\eta$ regions.
for the \LCWJES{} (full line) and \GCWJES{} (dashed line) calibration schemes. 
These are derived from a  combination of the \insitu{} techniques. 
The fractional \JES{} uncertainty for \EMJES{} derived from single hadrons response measurements
and systematic Monte Carlo simulation is overlaid in the shaded area for comparison.
For $\etajet > 1.2$ the $\eta$-intercalibration is shown as open symbols
for each jet calibration scheme.
\label{fig:insitucomparisonr4}}
\end{center}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> jetuncertaintyinsitucellweightingfiguresr4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htp]
\begin{center}
\subfloat[\GCWJES]{\includegraphics[width=0.49\textwidth]{InSituCombination/combined_TSpline1_GJ-TJ-MJB_GCW_R4_eta5_bins.eps}}
\subfloat[\LCWJES]{\includegraphics[width=0.49\textwidth]{InSituCombination/combined_TSpline1_GJ-TJ-MJB_LC_R4_eta5_bins.eps}}
%
\caption{Jet response ratio of the data and the Monte Carlo simulation
as a function of \ptjet{}
for three \insitu{} techniques using a reference objects
photons ($\gamma$-jet), a system of low energetic jets (multijet)
or the transverse momentum of all tracks associated to jets
(tacks in jets). The error bar displays the statistical and systematic
uncertainties added in quadrature.
Shown are the results for \antikt{} jets with $R = 0.4$
calibrated with the \GCWJES{} (a) and the \LCWJES{} (b) calibration scheme.
The green band indicates the combination of the \insitu{} techniques.
\label{fig:responseratioinsitucellweightingr4}}
\end{center}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[ht!p]
\begin{center}
\subfloat[\GCWJES]{\includegraphics[width=0.49\textwidth]{InSituCombination/Weights_TSpline1_GCW_R4_eta5.eps}}
\subfloat[\LCWJES]{\includegraphics[width=0.49\textwidth]{InSituCombination/Weights_TSpline1_LC_R4_eta5.eps}}
%
\caption{Weight carried by each \insitu{} technique in the combination to
derive the jet energy scale uncertainty for \antikt{} jets with $R = 0.4$ 
for $|\etajet| < 1.2$ calibrated with the
\GCWJES{} (a) and the \LCWJES{} (b) calibration scheme.
\label{fig:weightinsitucellweightingr4}}
\end{center}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[ht!p]
\begin{center}
\subfloat[\GCWJES]{\includegraphics[width=0.49\textwidth]{InSituCombination/Syst_TSpline1_combined_GCW_R4_eta5_bins.eps}}
\subfloat[\LCWJES]{\includegraphics[width=0.49\textwidth]{InSituCombination/Syst_TSpline1_combined_LC_R4_eta5_bins.eps}}
%
\caption{Jet energy scale uncertainty (solid line) for 
for \antikt{} jets with $R = 0.4$ for $|\etajet| < 1.2$ calibrated with the
\GCWJES{} (a) and the \LCWJES{} (b) calibration scheme.
The dashed line shows the JES uncertainty that could have been achieved,
if \insitu{} techniques had been used to recalibrate the jets.
\label{fig:uncertaintyinsitucellweightingr4}}
\end{center}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> jetuncertaintyinsitufiguresr04.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht!]
\begin{center}
%Subfloats
\includegraphics[width=0.49\textwidth]{InSituCombination/combined_TSpline1_GJ-TJ-MJB_JES_R4_eta5_bins.eps}
%
\caption{Jet response ratio of the data and the Monte Carlo simulation 
for $|\eta|<1.2$ as a function of \ptjet{}
for three \insitu{} techniques.
The error displays the statistical and systematic
uncertainties added in quadrature.
Shown are the results for \antikt{} jets with $R = 0.4$
calibrated with the \EMJES{} scheme.
The light band indicates the total uncertainty
from the combination of the \insitu{} techniques.
The inner dark band indicates the statistical component.
\label{fig:responseratioinsitur4}}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht!]
\begin{center}
%Subfloats
\subfloat[]{\includegraphics[width=0.49\textwidth]{InSituCombination/Weights_TSpline1_JES_R4_eta5.eps}}
%
\caption{
Weight carried by each \insitu{} technique in the combination to derive the jet energy scale uncertainty 
for \antikt{} jets with $R = 0.4$ calibrated with the \EMJES{} scheme.
\label{fig:weightinsitur4}}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht!]
\begin{center}
\includegraphics[width=0.49\textwidth]{InSituCombination/Syst_TSpline1_combined_JES_R4_eta5_bins.eps}
%
\caption{Jet energy scale uncertainty (solid line) for for \antikt{} jets 
with $R = 0.4$ calibrated with the \EMJES{} scheme for $|\eta|<1.2$.
The dashed line shows the JES uncertainty that could have been achieved,
if \insitu{} techniques had been used to recalibrate the jets.
The dark band indicates the JES uncertainties as derived from
the single hadron response measurements and Monte Carlo variation 
for $|\etajet|<0.3$.
\label{fig:uncertaintyinsitur4}}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%

